On-Board Vision-Language Models for Personalized Autonomous Vehicle Motion Control: System Design and Real-World Validation

Personalized driving refers to an autonomous vehicle's ability to adapt its driving behavior or control strategies to match individual users' preferences and driving styles while maintaining safety and comfort standards. However, existing works either fail to capture every individual preference precisely or become computationally inefficient as the user base expands. Vision-Language Models (VLMs) offer promising solutions to this front through their natural language understanding and scene reasoning capabilities. In this work, we propose a lightweight yet effective on-board VLM framework that provides low-latency personalized driving performance while maintaining strong reasoning capabilities. Our solution incorporates a Retrieval-Augmented Generation (RAG)-based memory module that enables continuous learning of individual driving preferences through human feedback. Through comprehensive real-world vehicle deployment and experiments, our system has demonstrated the ability to provide safe, comfortable, and personalized driving experiences across various scenarios and significantly reduce takeover rates by up to 76.9%. To the best of our knowledge, this work represents the first end-to-end VLM-based motion control system in real-world autonomous vehicles.

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

The autonomous driving industry is experiencing an evolution towards human-centric systems~\cite{calvert2020human,lou2024human}, where vehicle automation extends beyond only considering traditional safety and efficiency metrics but also considers understanding users' implicit instructions and providing personalized driving experiences. This trend reflects a growing recognition that successful adoption of the autonomous vehicle requires not just technically self-driving, but also the ability to provide human-like driving experiences that align with individual preferences and expectations~\cite{cui2024personalizedautonomousdrivinglarge,cui2024largelanguagemodelsautonomous}. Recent advances in human-centric autonomous driving have been significantly influenced by large language models (LLMs) and vision-language models (VLMs), which demonstrate strong capabilities in understanding and reasoning complex driving scenarios and implicit natural language instructions~\cite{luo2023valleyvideoassistantlarge,bai2023qwenvlversatilevisionlanguagemodel}. 

While these models have demonstrated remarkable capabilities in interpreting visual driving scenes~\cite{ma2023dolphinsmultimodallanguagemodel, Park_2024_WACV} and generating corresponding high-level policies~\cite{ma2024lampilot}, they face several critical limitations. First, the strong reasoning capabilities required for autonomous driving tasks leverage `large' LLMs or VLMs, as smaller models often lack sufficient reasoning and understanding abilities~\cite{stolfo2023causalframeworkquantifyrobustness}. However, the computational demands of these large-scale models make on-board deployment infeasible, forcing reliance on cloud-based large models. This solution introduces significant latency issues in the inference process, with response times reaching up to 3 or 4 seconds~\cite{pmlr-v202-liu23am}, making it incompatible with the near real-time requirements of autonomous driving. Moreover, the dependency on internet connectivity causes these systems to not work in areas with poor or no network coverage. Second, there remains a significant gap in research exploring the utilization of VLMs for enhancing control policies or adapting them to individual driving preferences and styles. This limitation is because of the inherent challenge of developing personalized autonomous systems that can accommodate diverse human driving behaviors while maintaining safety and efficiency. Furthermore, the gap between understanding individual driving preferences and translating them into actionable control policies remains a significant challenge. While some recent works have explored the use of natural language interfaces for vehicle control~\cite{sha2023languagempc,long2024vlm}, they typically lack the ability to maintain consistent personalization across different driving scenarios and conditions, and current research works do not have real-world validation.


To address these limitations, we propose an efficient on-board VLM-based framework that enables nearly real-time personalization of autonomous vehicle motion control while maintaining strong instruction and scene reasoning capabilities for our task, we conduct the successful end-to-end implementation of this VLM-based motion control system in a real-world vehicle, which is the \textbf{first of its kind} to the best of our knowledge. We leverage a lightweight yet effective vision-language model that can be deployed directly on vehicles while maintaining comparable reasoning capabilities to cloud-based solutions to provide reliable and personalized driving experience.  The main contributions of this work are summarized as follows:

\begin{itemize}
\item We propose a novel framework that leverages a small-scale fine-tuned on-board VLM to generate personalized reliable control strategies for autonomous vehicles instantaneously, which address critical computational constraints in autonomous vehicles and are independent of internet connectivity.
\item We introduce a RAG-based memory module that incorporates human feedback, enabling continuous learning and adaptation to provide personalized driving experiences.
\item We validate our system's effectiveness through comprehensive real-world vehicle deployment and experiments, demonstrating both reliable and trustworthy autonomous driving performance for all level of instructions (from explicit `go faster.' to implicit `I feel uncomfortable.'), and successful personalization capabilities by reducing the takeover rate up to 76.9\%.
\end{itemize}


% To address these limitations, we propose an efficient on-board VLM-based framework that enables nearly real-time personalization of autonomous vehicle motion control while maintaining strong reasoning capabilities for our task, we conduct the successful end-to-end implementation of this VLM-based motion control system in a real-world vehicle, which is the \textbf{first of its kind} to the best of our knowledge. We leverage a lightweight yet effective vision-language model that can be deployed directly on vehicles while maintaining comparable reasoning capabilities to cloud-based solutions. Additionally, an adaptive perception-instruction-control mapping that dynamically adjusts to individual driving styles through a Retrieval-Augmented Generation (RAG)-based memory module. The on-board VLMs address critical computational constraints in autonomous vehicles, including near real-time response requirements (maintaining latency around 1s), independence from internet connectivity, and our memory module solving the need for adaptation to changing driver preferences, all while operating within the safety and comfort requirements. The main contributions of this work are summarized as follows:
% \begin{itemize}
% \item We propose a novel framework that leverages a small-scale fine-tuned on-board VLM to generate personalized control strategies for autonomous vehicles.
% % \item We create 10k image-instruction-action pairs dataset based on Nuscene dataset to fine-tune our VLM to improve the reasoning ability for our task.
% \item We introduce a RAG-based memory module that incorporates human feedback, enabling continuous learning and adaptation to provide personalized driving experiences.
% \item We validate our system's effectiveness through comprehensive real-world vehicle deployment and experiments, demonstrating both reliable autonomous driving performance and successful personalization capabilities.
% \end{itemize}

==> sec/5_application.tex <==
\section{Applications and Discussion}
\label{sec:appli}
% Our personalized motion control system has already been proved to have significant capacity in providing reliable, comfortable and personalized control strategy. This is the first of its kind to leverage the VLMs into a practical product that helps the autonomous driving industry provide more human-centric, personalized, and human-like driving experiences. 

Our personalized motion control system has demonstrated significant capabilities in delivering reliable, comfortable, and personalized control strategies. This work is the first of its kind to successfully integrate VLMs into a practical autonomous driving system that can help the industry toward more human-centric and personalized driving experiences. We see several main contributions that can benefit from our solution:

\begin{itemize}
    \item \textit{Personalization} Our system demonstrates a remarkable ability to adapt to individual driving preferences or communication styles over time. Through the RAG-based memory module, the system can effectively learn user preferences from previous interactions and human feedback, from comfort-oriented driving with smoother accelerations to more aggressive driving styles. For instance, when receiving feedback like ``I prefer keeping larger acceleration" the system adjusts its control parameters accordingly while maintaining safety standards. This personalization extends to various driving scenarios, including lane-changing behavior, turning performance, and acceleration profiles.
    
    \item \textit{Instruction and Scene Understanding} Our fine-tuned VLM-based framework demonstrates reasoning and understanding capabilities by processing both visual scene information and natural language instructions, effectively bridging the gap between human intent, environmental context, and vehicle control. The system can interpret complex instructions within the current visual context - for instance, when a user says `drive more cautiously,' the system analyzes both the instruction and the current scene (such as a crowded street or adverse weather conditions) to adjust its behavior appropriately. This multimodal understanding enables robust performance across various scenarios, enhancing more intuitive and context-aware human-vehicle interaction.
    
    \item \textit{Efficiency} Our solution achieves siginificant computational efficiency through our optimized 8B VLM implementation. The system runs effectively on standard vehicle hardware without requiring high-end GPUs, making it suitable for commercial vehicle deployment. We achieve an average latency of 1.6 seconds for instruction processing and control strategy generation while maintaining modest GPU memory consumption of 20 GB, meeting real-world autonomous driving requirements.
\end{itemize}


% During our real-world validation, we still identified some notable challenges when utilizing VLM in autonomous control progress. 
% TBD

==> tab/hf_example.tex <==
%routes_testing_03_02_23_44_23 0155
\begin{table}[t!]\centering
\begin{minipage}{1.0\columnwidth}\vspace{0mm}    
\centering
\begin{tcolorbox} 
\centering
\footnotesize
\begin{tabular}{p{1.0\columnwidth} c}
\TBlack{ {\bf System Message ($\mathbf{S_0}$)} } &\\
You are an AI system for an autonomous vehicle, and a figure of the current outside view will be sent to you. \\
You need to analyze the image and the command from the driver and send back the appropriate controller's parameter values to the vehicle's control system.

Here are the parameters that you can adjust to create the controller action matrix: \textbf{[omitted]}\\
Here are some principles that you need to keep in mind when you are tuning the parameters: \textbf{[omitted]} \\
% Here are the APIs you can use: ... \textbf{[omitted]} \\
% I will give you \\
% Command: ... \\
% Context: ... \\
% You should then respond to me with \\
% Plan: How to complete the task step by step. \\
% Code: \\
%     1) Write a function taking NO argument. \\
%     2) Only use the APIs that I provided. \\
% ... [omitted]
\TBlack{ {\bf Instruction ($\mathbf{I_0}$)} } &\\
I would like to drive faster than now.\\
\TBlack{ {\bf Image Input ($\mathbf{V_0}$)} } &\\ 
\textbf{[omitted]} \\
\TBlack{ {\bf History Memory ($\mathbf{H_0}$)} } &\\
\textit{(Empty because no previous interaction)}\\

\hrulefill & \\
\TBlue{ {\bf Action Policies ($\mathbf{P_0}$)} } &\\
$K_p$ = 1.2 .. \textit{other parameters in the matrices are omitted.}
% $\begin{bmatrix}
%     1.2 (\textcolor{red}{K_p}) & 0 & 0.1 \\
%     ... & ... & ...
% \end{bmatrix}$
\vspace{1mm}

\TBlue{{\bf Human Feedback ($\mathbf{F_0}$)}} &\\
I still feel not fast enough, you may increase acceleration. \\

\vspace{-1mm}

\hrulefill & \\
\TBlack{$\mathbf{S_{1}}$,$\mathbf{V_{1}}$ are omitted} \\
\TBlack{ {\bf Human Instruction ($\mathbf{I_{1}}$)} } &\\
I am in a hurry. \\
\TBlack{{\bf History Memory ($\mathbf{H_1}$)} } &\\
Instruction: I would like to drive faster than now. \\
Scene Description: ... \\
\vspace{0.5mm}
Action: $\begin{bmatrix}
    1.2 (\textcolor{red}{K_p}) & 0 & 0.1 \\
     & ... & 
\end{bmatrix}$ \\
\vspace{0.5mm}
Human Feedback: I still feel not fast enough, you may increase acceleration. \\
\hrulefill & \\
\TBlue{ {\bf Action Policies ($\mathbf{P_1}$)} } &\\
$K_p$ = 1.5 ... \textit{other parameters in the matrices are omitted.}
% $\begin{bmatrix}
%     1.5 (\textcolor{red}{K_p}) & 0 & 0.1 \\
%      & ... & 
% \end{bmatrix}$
\vspace{1mm}
\\

\TBlue{{\bf Human Feedback ($\mathbf{F_1}$)}} &\\
I feel good about this trip. \\
\vspace{-1mm}

\end{tabular}
\vspace{-3mm}
\end{tcolorbox}
\caption{This example illustrates the reasoning process of the proposed framework.}





\label{tab:full_example}
\end{minipage}
\vspace{-5mm}
\end{table}

==> tab/hf_example_back.tex <==
%routes_testing_03_02_23_44_23 0155
\begin{table*}[t!]\centering
\begin{minipage}{1.0\linewidth} 
\centering
\begin{tcolorbox} 
\centering
\footnotesize
\begin{tabular}{p{0.97\columnwidth} c}
\TBlack{ {\bf System Message ($\mathbf{X_{sys}^{0}}$)} } \\
% You are a helpful assistant who writes Python code to complete any autonomous driving \\task specified by me.
% Here are the APIs you can use: ... [omitted]\\
\scriptsize
You are a helpful assistant that writes python code to complete any autonomous driving task specified by me. \\
\scriptsize
Here are the APIs you can use: \{apis\} \\
\scriptsize
Here are some useful programs written with the provided APIs: \{programs\} \\
\scriptsize
At each round of conversation, I will give you \\
\scriptsize
Code from last round: ... Command: ... Context: ... Feedback: ... \\
\scriptsize
You should then respond to me with \\
\scriptsize
Explain (if applicable): Are there any steps missing in your plan? Why is the code not satisfactory? \\
\scriptsize
Plan: How to complete the task step by step. \\
\scriptsize
Code: 1) Write a function taking NO argument. 2) Only use the APIs that I provided. 3) Anything defined outside a function will be ignored, define all your variables inside your functions. 4) Name your function in a meaningful way (considering both command and context). 5) You should only write one function, which will be called by me. Do not write multiple functions. 6) When calling `proceed()' or `stop()' function, you should always `yield' the return value of the function. 7) You can reuse the above useful programs. 8) Do not write infinite loops. 9) Do not use any constant from the context, as it may dynamically change. Call the APIs to get the latest values. 10) Always provide feedback to the user using the `say' function. \\
\scriptsize
You should only respond in the format as described below: \{response\_format\} \\

\TRed{ {\bf Instruction ($\mathbf{X_{q}^{0}}$)} } &\\
Take a left at the next light. \\
\TBlack{ {\bf Driving Context ($\mathbf{X_{c}^{0}}$)} } &\\
There is a traffic light and it is Red. It is 5.52 m ahead. My current speed is 7.0 m/s. There are no obstacles in the vicinity.
 \\
%\hrulefill & \\
\TBlue{ {\bf Chain-of-Thought Reasoning ($\mathbf{X_{r}^{0}}$) } } &\\
1) First, check the status of the traffic light. If it's red, the vehicle should stop before the intersection.
2) Once the traffic light turns green, the vehicle should prepare to take a left turn at the intersection.
3) The vehicle will then turn left at the next intersection.
4) Throughout the process, provide feedback to the passenger about what actions the vehicle is planning to take.
\\
\TBlue{ {\bf Code as Policies ($\mathbf{X_{p}^{0}}$)} } &\\
\vspace{-2mm}
TBD
% \begin{python}
% def take_left_at_next_light():
%     if check_red_light():
%         yield stop()
%         say("Stopping for the red light.")
%     say("The light is green now. Preparing to take a left turn.")
%     turn_left_at_next_intersection()
%     say("Taking a left turn at the intersection.")
%     yield proceed(check_speed_limit())
% \end{python}


\hrulefill & \\

\TRed{ {\bf Human Feedback ($\mathbf{X_{f}^{1}}$)} } &\\
You should have slowed down a little bit while making turns.

\TBlue{ {\bf Explanation ($\mathbf{X_{r}^{1}}$)} } &\\
Reducing the speed slightly below the speed limit during a turn can enhance safety, especially in autonomous driving scenarios where precise control is crucial for both passenger comfort and safety.\\

\TBlue{ {\bf Code as Policies ($\mathbf{X_{p}^{1}}$)} } &\\
\vspace{-2mm}
TBD
% \begin{python}
% # ... [omitted]
% # Reduce speed by a small factor (e.g., 90% of the speed limit) to ensure a safer turn
% safe_turn_speed = check_speed_limit() * 0.9
% # ... [omitted]
% yield proceed(safe_turn_speed)
% \end{python}

\hrulefill & \\

\TRed{ {\bf Human Feedback ($\mathbf{X_{f}^{2}}$)} } &\\
The turning speed was too fast.

\TBlue{ {\bf Explanation ($\mathbf{X_{r}^{2}}$)} } &\\
It appears that the safe turning speed calculated as 90\% of the speed limit was too fast for a safe left turn. To address this, we can further reduce the target speed for the turn to ensure safety.\\

\TBlue{ {\bf Code as Policies ($\mathbf{X_{p}^{2}}$)} } &\\
\vspace{-2mm}
\begin{python}
# ... [omitted]
# Reduce the speed to 70% of the speed limit for a safer turn
safe_turn_speed = check_speed_limit() * 0.7 
# ... [omitted]
\end{python}
\vspace{-2mm}


\end{tabular}
\end{tcolorbox}
\vspace{-2mm}
\caption{
This example illustrates the reasoning and code generation process of the proposed programming planner. The three blocks indicate that the generations occur in different iterations. Content with \TBlue{blue} titles (chain-of-thought reasoning, explanation, and code as policies) is generated by LLMs. Content with \TRed{red} titles (instruction and human feedback) is provided by humans. The initial prompt includes three components: a system message ($\xsys$), human instruction ($\xq$), and the current driving context ($\xc$). Subsequent prompts also include human feedback ($\xf$) and the policy code ($\xp$) from the last round. For brevity, the system message, human instruction, driving context, and code from the last round are not included in subsequent prompts. %Note that the visual image is not used to prompt GPT. It is included here for reference only.
}
\label{tab:full_example}
\end{minipage}
\end{table*}
